Relations de Hodge--Riemann et combinatoire des matro\"ides (d'apr\`es K. Adiprasito, J. Huh et E. Katz)

Finite matroids are combinatorial structures that express the concept of linear independence. In 1964, G.-C. Rota conjectured that the coefficients of the "characteristic polynomial" of a matroid $M$, polynomial whose coefficients enumerate its subsets of given rank, form a log-concave sequence. K. Adiprasito, J. Huh et E. Katz have proved this conjecture using methods which, although entirely combinatorial, are inspired by algebraic geometry. From the Bergman fan of the matroid $M$, they define a graded "Chow ring" $A(M)$ for which they prove analogs of the Poincar\'e duality, the Hard Lefschetz theorem, and the Hodge--Riemann relations. The sought for log-concavity inequalities are then analogous to the Khovanskii--Teissier inequalities.

==> frenchbst.tex <==
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{\'editeurs}        \def\bbleds{\'eds.}
\def\bbleditor{\'editeur}          \def\bbled{\'ed.}
\def\bbledby{\'edit\'e by}
\def\bbledition{\'edition}        \def\bbledn{\'ed.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n\textsuperscript o}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{p.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Pr\'epublication}
\def\bbltechrep{Pr\'ep.}
\def\bblmthesis{M\'emoire de DEA}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1\textsuperscript{re}}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\textsuperscript{e}}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\textsuperscript{e}}
\def\bblfourth{Fourth}          \def\bblfourtho{4\textsuperscript{e}}
\def\bblfifth{Fifth}            \def\bblfiftho{5\textsuperscript{e}}
\def\bblst{\textsuperscript{re}}
  \def\bblnd{\textsuperscript{e}}  \def\bblrd{\textsuperscript{e}}
\def\bblth{\textsperscript{e}}
\def\bbljan{Janvier}  \def\bblfeb{F\'evrier}  \def\bblmar{Mars}
\def\bblapr{Avril}    \def\bblmay{Mai}       \def\bbljun{Juin}
\def\bbljul{Juillet}     \def\bblaug{Ao\^ut}    \def\bblsep{Septembre}
\def\bbloct{Octobre}  \def\bblnov{Novembre}  \def\bbldec{Decembre}


